Constitutional adapters: Inference-time interventions for misalignment and misuse

Training models to act in accordance with an explicitly defined set of principles, or "constitution," has shown promise as a robust and transparent mechanism for AI alignment. However, the generality and flexibility of such methods remain unclear. Here, we show that constitution-consistent behavior can be distilled from synthetic corpora into lightweight objects (low-rank adapters and steering vectors). Despite never seeing a harmful request or jailbreak during training, such objects increase jailbreak defense success and measured alignment -- particularly at long context lengths and against multi-turn attacks, where they outperform both prompted and steered baselines. Subtracting control-trained from constitution-trained objects further accentuates these effects, yielding defenses we call "constitutional adapters" (CAs). CAs can be trained on a base model, transferred zero-shot to its post-trained checkpoint, and scaled at inference time to predictably trade off defense for benign compliance. Taken together, these results recommend CAs as a lightweight, portable, and tunable lever for mitigating misalignment and misuse in API deployments.

==> figures/fig7/fig7.tex <==
\begin{table}[ht]
\caption{Static rungs drawn on the Qwen3.5-4B robustness frontier.}
\label{tab:qwen-frontier-static}
\begin{center}
\begin{tabular}{lllll}
\multicolumn{1}{c}{\bf ARM}  &\multicolumn{1}{c}{\bf SEED}  &\multicolumn{1}{c}{\bf DOSE}  &\multicolumn{1}{c}{\bf $\Delta$ DEFENSE}  &\multicolumn{1}{c}{\bf $\Delta$ COMPLIANCE}
\\ \hline \\
\emph{unsteered (absolute)} &-- &-- &$66.2$ &$65.7$ \\
Refusal steer &-- &$0.15$ &$+13.0$ &$-8.5$ \\
Refusal steer &-- &$0.3$ &$+24.2$ &$-15.4$ \\
Refusal steer &-- &$0.5$ &$+32.9$ &$-26.7$ \\
Safety SI &-- &$1$ &$+21.9$ &$-6.7$ \\
Safety SI &-- &$1$ &$+10.0$ &$-7.4$ \\
Constitution SI &-- &$1$ &$+23.9$ &$-4.5$ \\
Constitution SI &-- &$1$ &$+23.6$ &$-4.1$ \\
Constitution SI &-- &$1$ &$+8.7$ &$-4.4$ \\
Difference ReLU steer &s1 &$0.5$ &$+9.4$ &$-10.8$ \\
Difference ReLU steer &s2 &$0.5$ &$+16.9$ &$-14.1$ \\
Difference ReLU steer &s3 &$0.5$ &$+15.6$ &$-13.6$ \\
Difference ReLU steer &s1 &$0.75$ &$+7.2$ &$-8.8$ \\
Difference ReLU steer &s2 &$0.75$ &$+18.9$ &$-16.5$ \\
Difference ReLU steer &s3 &$0.75$ &$+27.7$ &$-22.2$ \\
Difference ReLU steer &s1 &$1$ &$+12.8$ &$-6.2$ \\
Difference ReLU steer &s2 &$1$ &$+24.2$ &$-18.8$ \\
Difference ReLU steer &s3 &$1$ &$+31.2$ &$-28.3$ \\
Difference ReLU steer &s1 &$1.25$ &$+16.9$ &$-38.2$ \\
Difference ReLU steer &s2 &$1.25$ &$+27.3$ &$-23.5$ \\
Difference ReLU steer &s3 &$1.25$ &$+33.1$ &$-46.6$ \\
Difference LoRA &s1 &$0.5$ &$+25.7$ &$-7.8$ \\
Difference LoRA &s2 &$0.5$ &$+20.9$ &$+1.5$ \\
Difference LoRA &s3 &$0.5$ &$+28.0$ &$-7.9$ \\
Difference LoRA &s1 &$0.75$ &$+29.6$ &$-10.0$ \\
Difference LoRA &s2 &$0.75$ &$+28.0$ &$+0.9$ \\
Difference LoRA &s3 &$0.75$ &$+32.3$ &$-16.2$ \\
Difference LoRA &s1 &$1$ &$+30.5$ &$-8.2$ \\
Difference LoRA &s2 &$1$ &$+28.9$ &$-7.5$ \\
Difference LoRA &s3 &$1$ &$+32.6$ &$-18.5$ \\
Difference LoRA &s1 &$1.25$ &$+31.7$ &$-10.7$ \\
Difference LoRA &s3 &$1.25$ &$+32.4$ &$-17.6$ \\
\end{tabular}
\end{center}
\end{table}

\begin{table}[ht]
\caption{Multi-turn rungs drawn on the Qwen3.5-4B robustness frontier.}
\label{tab:qwen-frontier-multi-turn}
\begin{center}
\begin{tabular}{lllll}
\multicolumn{1}{c}{\bf ARM}  &\multicolumn{1}{c}{\bf SEED}  &\multicolumn{1}{c}{\bf DOSE}  &\multicolumn{1}{c}{\bf $\Delta$ DEFENSE}  &\multicolumn{1}{c}{\bf $\Delta$ COMPLIANCE}
\\ \hline \\
\emph{unsteered (absolute)} &-- &-- &$2.9$ &$65.7$ \\
Refusal steer &-- &$0.15$ &$+1.3$ &$-8.5$ \\
Refusal steer &-- &$0.3$ &$+7.5$ &$-15.4$ \\
Refusal steer &-- &$0.5$ &$+33.1$ &$-26.7$ \\
Safety SI &-- &$1$ &$+2.8$ &$-6.7$ \\
Safety SI &-- &$1$ &$+4.4$ &$-7.4$ \\
Constitution SI &-- &$1$ &$+1.9$ &$-4.4$ \\
Difference ReLU steer &s1 &$0.5$ &$+0.4$ &$-10.8$ \\
Difference ReLU steer &s2 &$0.5$ &$+3.3$ &$-14.1$ \\
Difference ReLU steer &s3 &$0.5$ &$+3.1$ &$-13.6$ \\
Difference ReLU steer &s1 &$0.75$ &$+4.1$ &$-8.8$ \\
Difference ReLU steer &s2 &$0.75$ &$+11.8$ &$-16.5$ \\
Difference ReLU steer &s3 &$0.75$ &$+9.3$ &$-22.2$ \\
Difference ReLU steer &s1 &$1$ &$+15.8$ &$-6.2$ \\
Difference ReLU steer &s2 &$1$ &$+32.4$ &$-18.8$ \\
Difference ReLU steer &s3 &$1$ &$+40.7$ &$-28.3$ \\
Difference ReLU steer &s1 &$1.25$ &$+53.7$ &$-38.2$ \\
Difference ReLU steer &s2 &$1.25$ &$+56.0$ &$-23.5$ \\
Difference ReLU steer &s3 &$1.25$ &$+71.6$ &$-46.6$ \\
Difference LoRA &s1 &$0.5$ &$+4.2$ &$-7.8$ \\
Difference LoRA &s2 &$0.5$ &$+3.8$ &$+1.5$ \\
Difference LoRA &s3 &$0.5$ &$+10.7$ &$-7.9$ \\
Difference LoRA &s1 &$0.75$ &$+13.3$ &$-10.0$ \\
Difference LoRA &s2 &$0.75$ &$+12.5$ &$+0.9$ \\
Difference LoRA &s3 &$0.75$ &$+32.2$ &$-16.2$ \\
Difference LoRA &s1 &$1$ &$+24.1$ &$-8.2$ \\
Difference LoRA &s2 &$1$ &$+25.0$ &$-7.5$ \\
Difference LoRA &s3 &$1$ &$+41.1$ &$-18.5$ \\
Difference LoRA &s1 &$1.25$ &$+32.8$ &$-10.7$ \\
Difference LoRA &s3 &$1.25$ &$+43.0$ &$-17.6$ \\
\end{tabular}
\end{center}
\end{table}
